A survey of electricity spot and futures price models for risk management applications

This review presents the set of electricity price models proposed in the literature since the opening of power markets. We focus on price models applied to financial pricing and risk management. We classify these models according to their ability to represent the random behavior of prices and some of their characteristics. In particular, this classification helps users to choose among the most suitable models for their risk management problems.

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions tr\`es usit\'ees
%
% Derniere modif le 10-07-96
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
\def\reff#1{\XS(\ref{#1})}
\def\refs#1{section~\ref{#1}}
\def\refS#1{Section~\ref{#1}}

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  
% Numéro (pour biblio)
\def\numero{n°}
\def\Numero{N°}

% Majuscules
\def\UP#1{\uppercase{#1}}       % majuscules
\def\up#1{\uppercase{#1}}       % majuscules

% Liste des abreges
\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-\`a-dire\XS}
\def\cad{c'est-\`a-dire\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vit\ae}\XS}
\def\Cv{\textit{Curriculum vit\ae}\XS}
\def\CV{\textit{Curriculum Vit\ae}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-\`a-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vit\ae}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}


\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}

\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}

\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}
\def\EEA{\'Electronique \'Electrotechnique Automatique\XS}
\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}
\def\ATS{Automatique et Traitement du Signal\XS}

\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}
\def\TE{travaux d'études\XS}
\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}
\def\TD{travaux dirigés\XS}
\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}
\def\TP{travaux pratiques\XS}
%\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\TDAO{travaux dirigés assistés sur ordinateur\XS}
\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\ts{traitement du signal\XS}
\def\TS{Traitement du Signal\XS}

\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}

\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}
% Operating Systemes 
\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% langages
\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

\def\crec{chargé de recherches\XS}
\def\Crec{Chargé de recherches\XS}
\def\dr{directeur de recherches\XS}
\def\Dr{Directeur de recherches\XS}


% congres
\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{C}{hampagnat}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Fr\'ed\'eric}{D}{ublanchet}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy Le}{B}{esnerais}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Herv\'e}{C}{arfantan}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{J\'er\^ome}{I}{dier}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{St\'ephane}{B}{rette}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}

% Acronymes et raccourcis
%
\def\ATER{Attach\'e temporaire d'enseignement et de recherche}
\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}
\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

\def\CdO{Centre d'Orsay\XS}

\def\CEA{Commissariat à l'\'Enegie Atomique\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}
\def\DRM{D\'epartement de Recherche M\'edicale\XS}
\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}
\def\DSV{Direction des Sciences du Vivant\XS}
\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}
\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
\def\SHFJ{Service Hospitalier Frédéric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\UNAF{Unit\'e de Neuroimagerie Anatomo Foncxtionnelle\XS}
\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}


\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}
\def\CHU{Centre Hospitalier Universitaire\XS}
\def\salpe{Salpétrière\XS}
\def\hsalpe{Hôpital de la Salpétrière\XS}
\def\pisalpe{Pitié-Salpétrière\XS}
\def\gpisalpe{Groupe Pitié-Salpétrière\XS}

\def\CNRS{Centre National de la Recherche Scientifique\XS}
\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}
\def\EDF{\'Electricité de France\XS}

\def\ENSTA{\'Ecole Nationale Sup\'erieure de Techniques Avanc\'ees\XS}
\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}
\def\ESIEA{\'Ecole Supérieure d'Informatique \'Electronique Automatique\XS}
\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}
\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}


\def\GPI{Groupe Probl\`emes Inverses\XS}
\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

\def\INSERM{Institut National pour la Sant\'e et la Recherche M\'edicale\XS}
\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

\def\CNAM{Conservatoire National des Arts et Métiers\XS}
\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

\def\IAS{Institut d'Astrophysique Spatiale\XS}
\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}
\def\IPSN{Institut de Protection et de Sureté Nucléaire\XS}

\def\LSS{Laboratoire des Signaux et Syst\`emes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}

\def\LIMSI{Laboratoire d'Informatique pour la Mécanique et les Sciences de l'Ingénieur\XS}
\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

\def\ONERA{Office National d'\'Etudes et de Recherches A\'erospatiales\XS}
\newcommand{\onera}[1][\scad]{\sca[#1]{on\'era}\XS}

\def\MDC{Ma\^\i tre de conf\'erences\XS}
\def\MDCs{Ma\^\i tres de conf\'erences\XS}
\newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

\newcommand{\UND}[1][\scad]{Université de Notre Dame, \sca[#1]{usa}\XS}

\def\UPS{Universit\'e Paris-Sud\XS}
\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
\newcommand{\upxi}[1][\scad]{\sca[#1]{upxi}\XS}

% Unites Thomson
\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Unite propre de recherche
\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}
% LENA, lena upr640,...
\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
% Nous
\def\GsY{Gif--sur--Yvette\XS}
\newcommand{\ESE}[1][\scad]{\sca[#1]{sup\'elec}\XS}

\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
%\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\hiercea}[1][\scad]{\dsv[#1]/\drm[#1]/\shfj[#1]\XS}

\newcommand{\adresse}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\adresscea}[1][\scad]{4 Place du Général Leclerc, 91406 Orsay Cedex, France\XS}
\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
%\newcommand{\tutelle}[1][\scad]{\sca[#1]{Cnrs~--~Sup\'elec~--~Ups}}
\def\ALSS{\LSS~(\tutelle)\\\adresse}
\def\ALSSun{\LSS (\tutelle) \adresse}
%


% ---------------------------------------------------- 
% Modele d'en-tete par A. Mohammad-Djafari et J. Idier 
% ---------------------------------------------------- 
%
\def\helvnormal#1{{\fontfamily{phv}\fontsize{11}{14pt}\selectfont #1}}
\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}
%
\newcommand{\entete}[5][Nom.Pr\'enom]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Supélec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique          \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
T\'el\'ephone\,: 01 69 85 17 12 --- 
T\'el\'ecopie\,: 01 69 85 17 65 --- 
Courriel\,: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/R\'ef.\,: #2} & \helvscript{\sca[-3]{Gif}, le} #5\\%
\helvscript{N/R\'ef.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inhead}[5][Name.Surname]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Supélec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique  \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYST\`EMES}}\\%
\helvfoot{Unit\'e mixte de recherche n$^{\rm o}$ 8506\\%
Sup\'elec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Telephone: 01 69 85 17 12 --- 
Fax: 01 69 85 17 65 --- 
E-mail: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Gif}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
} 



==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gauthiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}

% ALPHABET GRAS et Chapeau
\def\Abh{\hat{{\sbm{A}}}\XS}  \def\abh{\hat{{\sbm{a}}}\XS}
\def\Bbh{\hat{{\sbm{B}}}\XS}  \def\bbh{\hat{{\sbm{b}}}\XS}
\def\Cbh{\hat{{\sbm{C}}}\XS}  \def\cbh{\hat{{\sbm{c}}}\XS}
\def\Dbh{\hat{{\sbm{D}}}\XS}  \def\dbh{\hat{{\sbm{d}}}\XS}
\def\Ebh{\hat{{\sbm{E}}}\XS}  \def\ebh{\hat{{\sbm{e}}}\XS}
\def\Fbh{\hat{{\sbm{F}}}\XS}  \def\fbh{\hat{{\sbm{f}}}\XS}
\def\Gbh{\hat{{\sbm{G}}}\XS}  \def\gbh{\hat{{\sbm{g}}}\XS}
\def\Hbh{\hat{{\sbm{H}}}\XS}  \def\hbh{\hat{{\sbm{h}}}\XS}
\def\Ibh{\hat{{\sbm{I}}}\XS}  \def\ibh{\hat{{\sbm{i}}}\XS}
\def\Jbh{\hat{{\sbm{J}}}\XS}  \def\jbh{\hat{{\sbm{j}}}\XS}
\def\Kbh{\hat{{\sbm{K}}}\XS}  \def\kbh{\hat{{\sbm{k}}}\XS}
\def\Lbh{\hat{{\sbm{L}}}\XS}  \def\lbh{\hat{{\sbm{l}}}\XS}
\def\Mbh{\hat{{\sbm{M}}}\XS}  \def\mbh{\hat{{\sbm{m}}}\XS}
\def\Nbh{\hat{{\sbm{N}}}\XS}  \def\nbh{\hat{{\sbm{n}}}\XS}
\def\Obh{\hat{{\sbm{O}}}\XS}  \def\obh{\hat{{\sbm{o}}}\XS}
\def\Pbh{\hat{{\sbm{P}}}\XS}  \def\pbh{\hat{{\sbm{p}}}\XS}
\def\Qbh{\hat{{\sbm{Q}}}\XS}  \def\qbh{\hat{{\sbm{q}}}\XS}
\def\Rbh{\hat{{\sbm{R}}}\XS}  \def\rbh{\hat{{\sbm{r}}}\XS}
\def\Sbh{\hat{{\sbm{S}}}\XS}  \def\sbh{\hat{{\sbm{s}}}\XS}
\def\Tbh{\hat{{\sbm{T}}}\XS}  \def\tbh{\hat{{\sbm{t}}}\XS}
\def\Ubh{\hat{{\sbm{U}}}\XS}  \def\ubh{\hat{{\sbm{u}}}\XS}
\def\Vbh{\hat{{\sbm{V}}}\XS}  \def\vbh{\hat{{\sbm{v}}}\XS}
\def\Wbh{\hat{{\sbm{W}}}\XS}  \def\wbh{\hat{{\sbm{w}}}\XS}
\def\Xbh{\hat{{\sbm{X}}}\XS}  \def\xbh{\hat{{\sbm{x}}}\XS}
\def\Ybh{\hat{{\sbm{Y}}}\XS}  \def\ybh{\hat{{\sbm{y}}}\XS}
\def\Zbh{\hat{{\sbm{Z}}}\XS}  \def\zbh{\hat{{\sbm{z}}}\XS}

\def\alphabh      {\hat{{\sbmm{\alpha}}}\XS}
\def\betabh       {\hat{{\sbmm{\beta}}}\XS}
\def\gammabh      {\hat{{\sbmm{\gamma}}}\XS}      \def\Gammabh    {\hat{{\sbmm{\Gamma}}}\XS}
\def\deltabh      {\hat{{\sbmm{\delta}}}\XS}      \def\Deltabh    {\hat{{\sbmm{\Delta}}}\XS}
\def\epsilonbh    {\hat{{\sbmm{\epsilon}}}\XS}
\def\varepsilonbh {\hat{{\sbmm{\varepsilon}}}\XS}
\def\etabh        {\hat{{\sbmm{\eta}}}\XS}
\def\thetabh      {\hat{{\sbmm{\theta}}}\XS}      \def\Thetabh    {\hat{{\sbmm{\Theta}}}\XS}
\def\varthetabh   {\hat{{\sbmm{\vartheta}}}\XS}
\def\iotabh       {\hat{{\sbmm{\iota}}}\XS}
\def\kappabh      {\hat{{\sbmm{\kappa}}}\XS}
\def\varkappabh   {\hat{{\sbmm{\varkappa}}}\XS}
\def\lambdabh     {\hat{{\sbmm{\lambda}}}\XS}     \def\Lambdabh   {\hat{{\sbmm{\Lambda}}}\XS}
\def\mubh         {\hat{{\sbmm{\mu}}}\XS}
\def\nubh         {\hat{{\sbmm{\nu}}}\XS}
\def\xibh         {\hat{{\sbmm{\xi}}}\XS}         \def\Xibh       {\hat{{\sbmm{\Xi}}}\XS}
\def\pibh         {\hat{{\sbmm{\pi}}}\XS}         \def\Pibh       {\hat{{\sbmm{\Pi}}}\XS}
\def\varpibh      {\hat{{\sbmm{\varpi}}}\XS}
\def\rhobh        {\hat{{\sbmm{\rho}}}\XS}
\def\varrhobh     {\hat{{\sbmm{\varrho}}}\XS}
\def\sigmabh      {\hat{{\sbmm{\sigma}}}\XS}      \def\Sigmabh    {\hat{{\sbmm{\Sigma}}}\XS}
\def\varsigmabh   {\hat{{\sbmm{\varsigma}}}\XS}   \def\Varsigmabh {\hat{{\sbmm{\Varsigma}}}\XS}
\def\phibh        {\hat{{\sbmm{\phi}}}\XS}        \def\Phibh      {\hat{{\sbmm{\Phi}}}\XS}
\def\varphibh     {\hat{{\sbmm{\varphi}}}\XS}
\def\chibh        {\hat{{\sbmm{\chi}}}\XS}
\def\psibh        {\hat{{\sbmm{\psi}}}\XS}        \def\Psibh      {\hat{{\sbmm{\Psi}}}\XS}
\def\omegabh      {\hat{{\sbmm{\omega}}}\XS}      \def\Omegabh    {\hat{{\sbmm{\Omega}}}\XS}
\def\taubh        {\hat{{\sbmm{\tau}}}\XS}
\def\upsilonbh    {\hat{{\sbmm{\upsilon}}}\XS}   \def\Upsilonbh  {\hat{{\sbmm{\Upsilon}}}\XS}
\def\zetabh       {\hat{{\sbmm{\zeta}}}\XS}





% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS} 
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}

% ALPHABET GAUTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  \def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}

